Aspects g\'eom\'etriques et int\'egrables des mod\`eles de matrices al\'eatoires

This thesis deals with the geometric and integrable aspects associated with random matrix models. Its purpose is to provide various applications of random matrix theory, from algebraic geometry to partial differential equations of integrable systems. The variety of these applications shows why matrix models are important from a mathematical point of view. First, the thesis will focus on the study of the merging of two intervals of the eigenvalues density near a singular point. Specifically, we will show why this special limit gives universal equations from the Painlev\'e II hierarchy of integrable systems theory. Then, following the approach of (bi) orthogonal polynomials introduced by Mehta to compute partition functions, we will find Riemann-Hilbert and isomonodromic problems connected to matrix models, making the link with the theory of Jimbo, Miwa and Ueno. In particular, we will describe how the hermitian two-matrix models provide a degenerate case of Jimbo-Miwa-Ueno's theory that we will generalize in this context. Furthermore, the loop equations method, with its central notions of spectral curve and topological expansion, will lead to the symplectic invariants of algebraic geometry recently proposed by Eynard and Orantin. This last point will be generalized to the case of non-hermitian matrix models (arbitrary $\beta$) paving the way to "quantum algebraic geometry" and to the generalization of symplectic invariants to "quantum curves". Finally, this set up will be applied to combinatorics in the context of topological string theory, with the explicit computation of an hermitian random matrix model enumerating the Gromov-Witten invariants of a toric Calabi-Yau threefold.

==> FeuilleDegarde.tex <==
\thispagestyle{empty}
\selectlanguage{french}
\begin{center}
Université de Montréal
\\
et
\\
Université Paris-Diderot (Paris 7)
\end{center}

\medskip
\medskip
\medskip
\medskip



\begin{center}
\textbf{Aspects géométriques et intégrables des modèles de matrices aléatoires}
\end{center}

\medskip
\medskip
\medskip
\medskip




\begin{center}
par\\
Olivier Marchal
\end{center}

\medskip
\medskip
\medskip
\medskip
\medskip
\medskip



\begin{center}
Département de mathématiques et de statistique\\
Faculté des arts et des sciences\\
et\\
Institut de physique théorique\\
Commissariat à l'énergie atomique
\end{center}

\medskip
\medskip
\medskip
\medskip




\begin{center}
 Thèse présentée à la Faculté des études supérieures\\
en vue de l'obtention du grade de Philosophi\ae  Doctor (Ph.D.)\\
en mathématiques 
\end{center}


\medskip
\medskip
\medskip
\medskip
\medskip




\begin{center}
 Décembre, 2010
\end{center}

\medskip
\medskip
\medskip
\medskip




\begin{center}
 \copyright \, Olivier Marchal, 2010.
\end{center}



==> FeuilleDegarde2.tex <==
\thispagestyle{empty}
\selectlanguage{french}
\begin{center}
Université de Montréal
\\
Faculté des études supérieures
\\
et
\\
Université Paris-Diderot (Paris 7)

\end{center}

\medskip
\medskip
\medskip
\medskip
\medskip
\medskip

\begin{center}
Cette thèse intitulée:\\
\medskip

\textbf{Aspects géométriques et intégrables des modèles de matrices aléatoires} 
\end{center}




\medskip
\medskip
\medskip



\begin{center}
présentée par:
\\
Olivier Marchal
\end{center}

\medskip
\medskip
\medskip



\begin{center}
a été évaluée par un jury composé des personnes suivantes:\\
\medskip
\medskip
$\begin{array}{ll}
\text{St-Aubin Yvan - Université de Montréal}, & \text{président-rapporteur}\\
\text{Eynard Bertrand et Harnad John},& \text{directeurs de recherche}\\
%\text{John Harnad, }& \text{codirecteur}\\
\text{Bertola Marco - Université Concordia},& \text{membre du jury}\\ 
\text{Hurtubise Jacques - Université McGill},& \text{membre du jury}\\ 
\text{Zuber Jean-Bernard - Université Paris VI},& \text{examinateur externe}\\
\text{Paranjape Manu B}& \text{représentant du doyen de la FES}\\
\end{array}$
\end{center}

\medskip
\medskip
\medskip
\medskip
\medskip


\begin{center}
 Thèse acceptée le: 20 décembre 2010
\end{center}




==> dedicace.tex <==
 \dedicace
\selectlanguage{french}
  \vspace*{1.0cm}

   \hspace{2.5in}
    (A ma famille) 

